Extraction of the Coulomb Sum Rule, Transverse Enhancement, and Longitudinal Quenching from an Analysis of all Available e-$^{12}$C and e-$^{16}$O Cross Section Data

We report on a phenomenological analysis of all available electron scattering data on ${\rm ^{12}C}$ (about 6600 differential cross section measurements) and on ${\rm ^{16}O}$ (about 250 measurements) within the framework of the quasielastic (QE) superscaling model (including Pauli blocking). All QE and inelastic cross section measurements are included down to the lowest momentum transfer $\bf q$ (including photo-production data). We find that there is enhancement of the transverse QE response function ($R_T^{QE}$) and quenching of the QE longitudinal response function ($R_L^{QE}$) at low $\bf q$ (in addition to Pauli blocking). We extract parameterizations of a $multiplicative$ low $\bf q$ "Longitudinal Quenching Factor" and an $additive$ "Transverse Enhancement" contribution. Additionally, we find that the excitation of nuclear states contribute significantly (up to 30\%) to the Coulomb Sum Rule $SL({\bf q})$. We extract the most accurate determination of $SL({\bf q})$ to date and find it to be in reasonable agreement with recent theoretical calculations.

==> authors_inputs.tex <==
\newcommand{\Rochester}{Department of Physics and Astronomy, University of Rochester, Rochester, NY  14627, USA}
\newcommand{\JLAB}{Thomas Jeferson National Accelerator Facility, Newport News, VA 23606, USA}

==> authors_list.tex <==
\affiliation{\Rochester}
\affiliation{\JLAB}
  \author{A.~Bodek}
%   \thanks{Corresponding author  Arie Bodek, bodek@pas.rochester.edu}
\affiliation{\Rochester}
    \author{M.~E.~Christy}
\affiliation{\JLAB}
 %   christy@jlab.org
 % M. Eric Christy
 \
